Learning to Self-Train for Semi-Supervised Few-Shot Classification

Few-shot classification (FSC) is challenging due to the scarcity of labeled training data (e.g. only one labeled data point per class). Meta-learning has shown to achieve promising results by learning to initialize a classification model for FSC. In this paper we propose a novel semi-supervised meta-learning method called learning to self-train (LST) that leverages unlabeled data and specifically meta-learns how to cherry-pick and label such unsupervised data to further improve performance. To this end, we train the LST model through a large number of semi-supervised few-shot tasks. On each task, we train a few-shot model to predict pseudo labels for unlabeled data, and then iterate the self-training steps on labeled and pseudo-labeled data with each step followed by fine-tuning. We additionally learn a soft weighting network (SWN) to optimize the self-training weights of pseudo labels so that better ones can contribute more to gradient descent optimization. We evaluate our LST method on two ImageNet benchmarks for semi-supervised few-shot classification and achieve large improvements over the state-of-the-art method. Code is at https://github.com/xinzheli1217/learning-to-self-train.

==> 5_table_backbones.tex <==
\begin{table*}[!h]
% \left
%
\vspace{-6pt}
\small
\centering
\begin{tabular}{lcccccccc}
\toprule 
& \multicolumn{2}{c}{MAML~\cite{FinnAL17}}
&& \multicolumn{2}{c}{LEO~\cite{RusuICLR2019}}\\
\cmidrule{2-3}\cmidrule{5-6}
& mini(1-shot) / D & tiered / D  && mini / D & tiered / D\\
\midrule[1pt]
\midrule[1pt]
\emph{recursive,hard,soft} & 54.8 / 52.0 & 58.6 / 55.5  && 66.0 / 63.5  & 75.9 / 74.3 \\
TPN~\cite{LiuICLR2019transductive} & 52.8 / 50.4  & 55.7 / 53.5 && 62.7 / 61.3 &  72.1 / 71.5\\
\bottomrule[1pt]
\end{tabular}
\vspace{-0.15cm}
\caption{5-way, 1-shot classification accuracy ($\%$) by replacing our base network MTL(ResNet-12)~\cite{SunCVPR2019} with MAML(4CONV)~\cite{FinnAL17} and LEO(ResNet-12)~\cite{RusuICLR2019}.}
\label{table_backbones}
\end{table*}
